HBert + BiasCorp -- Fighting Racism on the Web

Subtle and overt racism is still present both in physical and online communities today and has impacted many lives in different segments of the society. In this short piece of work, we present how we're tackling this societal issue with Natural Language Processing. We are releasing BiasCorp, a dataset containing 139,090 comments and news segment from three specific sources - Fox News, BreitbartNews and YouTube. The first batch (45,000 manually annotated) is ready for publication. We are currently in the final phase of manually labeling the remaining dataset using Amazon Mechanical Turk. BERT has been used widely in several downstream tasks. In this work, we present hBERT, where we modify certain layers of the pretrained BERT model with the new Hopfield Layer. hBert generalizes well across different distributions with the added advantage of a reduced model complexity. We are also releasing a JavaScript library and a Chrome Extension Application, to help developers make use of our trained model in web applications (say chat application) and for users to identify and report racially biased contents on the web respectively.

==> faulty.tex <==

% Demographic Word Embeddings for Racism Detection on Twitter Mohammed Hasanuzzaman Gael Dias Andy Way Proceedings of the 8th International Joint Conference on Natural Language Processing, pages 926–936, Taipei, Taiwan, November 27 – December 1, 2017


% [Nockleby 2000] John T. Nockleby, Hate Speech. In
% Encyclopedia of the American Constitution (2nd ed.,
% edited by Leonard W. Levy, Kenneth L. Karst et al.,
% New York: Macmillan, 2000), pp. 1277-1279

% W. Warner and J. Hirschberg. 2012. Detecting Hate
% Speech on the World Wide Web. In Proceedings of
% the Second Workshop on Language in Social Media
% (LSM 2012), pages 19–26.




% @inproceedings{yahoo_nobata,
%   title={Distributed representations of geographically situated language},
%   author={David Bamman, Chris Dyer, and Noah A. Smith},
%   booktitle={Proceedings of the Association for Computational Linguistics},
%   pages={828–834},
%   year={2014},
% }



% greevy_2004_princip

% Text Categorisation of Racist Texts Using a Support Vector Machine Edel P. Greevy1 , Alan F. Smeaton
% JADT 2004 : 7es Journées internationales d’Analyse statistique des Données Textuelles


% Pete Burnap and Matthew L. Williams. 2016. Us and
% them: identifying cyber hate on twitter across multiple protected characteristics. EPJ Data Science,
% 5(1):11.

	
% Katharine Gelber and Adrienne Sarah Ackary Stone.
% 2007. Hate Speech and Freedom of Speech in Australia, volume 2118. Federation Press.	

% Detecting White Supremacist Hate Speech using Domain Specific Word Embedding with Deep Learning and BERT Hind Saleh, Areej Alhothali, Kawthar Moria 
% Information Processing and Management

